FairPilot: An Explorative System for Hyperparameter Tuning through the Lens of Fairness

Despite the potential benefits of machine learning (ML) in high-risk decision-making domains, the deployment of ML is not accessible to practitioners, and there is a risk of discrimination. To establish trust and acceptance of ML in such domains, democratizing ML tools and fairness consideration are crucial. In this paper, we introduce FairPilot, an interactive system designed to promote the responsible development of ML models by exploring a combination of various models, different hyperparameters, and a wide range of fairness definitions. We emphasize the challenge of selecting the ``best" ML model and demonstrate how FairPilot allows users to select a set of evaluation criteria and then displays the Pareto frontier of models and hyperparameters as an interactive map. FairPilot is the first system to combine these features, offering a unique opportunity for users to responsibly choose their model.

==> Tables.tex <==
% \begin{doc ument}



\begin{longtable} [c]{| c | c |}
% \begin{table}[h]
% \begin{tabular}[c]{| c | c |}
 \caption{Decision Tree: Hyperparameter Space.\label{dths}}\\

 \hline
 \multicolumn{2}{| c |}{Decision Tree}\\
 \hline
 Hyperparameter & Space\\
 \hline
 \endfirsthead

 \hline
 \multicolumn{2}{|c|}{Continuation of Table \ref{long}}\\
 \hline
 Something & something else\\
 \hline
 \endhead

 \hline
 \endfoot

 \hline
 \hline\hline
 \endlastfoot

 criterion & [gini, entropy]\\
 max features & [None, sqrt, log2]\\
 min samples split & [2, 4, 8, 12, 16, 20]\\
 min samples leaf & [1, 4, 8, 12, 16, 20]\\
 class weight & [None, balanced]\\
% \end{tabular}
%  \end{table}
\end{longtable}
 
 \begin{longtable}[c]{| c | c |}
 \caption{Random Forest, Hyperparameter Space.\label{rfhs}}\\

 \hline
 \multicolumn{2}{| c |}{Random Forest}\\
 \hline
 Hyperparameter & Space\\
 \hline
 \endfirsthead

 \hline
 \multicolumn{2}{|c|}{Continuation of Table \ref{long}}\\
 \hline
 Something & something else\\
 \hline
 \endhead

 \hline
 \endfoot

 \hline
 \hline\hline
 \endlastfoot

 criterion & [gini, entropy]\\
 max features & [None, sqrt, log2]\\
 min samples split & [2, 4, 8, 12, 16, 20]\\
 min samples leaf & [1, 4, 8, 12, 16, 20]\\
 class weight & [None, balanced]\\
 bootstrap & [False, True]\\
 \end{longtable}

 \begin{longtable}[c]{| c | c |}
 \caption{Logistic Regression, Hyperparameter Space.\label{lrhs}}\\

 \hline
 \multicolumn{2}{| c |}{Logistic Regression}\\
 \hline
 Hyperparameter & Space\\
 \hline
 \endfirsthead

 \hline
 \multicolumn{2}{|c|}{Continuation of Table \ref{long}}\\
 \hline
 Something & something else\\
 \hline
 \endhead

 \hline
 \endfoot

 \hline
 \hline\hline
 \endlastfoot

 C & [0.001, 0.01, 0.1, 1, 10, 100, 1000]\\
 penalty & [l2, none]\\
\end{longtable}

 \begin{longtable}[c]{| c | c |}
 \caption{SVC, Hyperparameter Space.\label{svchs}}\\

 \hline
 \multicolumn{2}{| c |}{Sequential Vector Classifier}\\
 \hline
 Hyperparameter & Space\\
 \hline
 \endfirsthead

 \hline
 \multicolumn{2}{|c|}{Continuation of Table \ref{long}}\\
 \hline
 Something & something else\\
 \hline
 \endhead

 \hline
 \endfoot

 \hline
 \hline\hline
 \endlastfoot

 C & [0.001, 0.01, 0.1, 1, 10, 100, 1000]\\
 kernel & [linear, poly, rbf, sigmoid]\\
\end{longtable}
 % \end{document}

